A Recommender System for Scientific Datasets and Analysis Pipelines

Scientific datasets and analysis pipelines are increasingly being shared publicly in the interest of open science. However, mechanisms are lacking to reliably identify which pipelines and datasets can appropriately be used together. Given the increasing number of high-quality public datasets and pipelines, this lack of clear compatibility threatens the findability and reusability of these resources. We investigate the feasibility of a collaborative filtering system to recommend pipelines and datasets based on provenance records from previous executions. We evaluate our system using datasets and pipelines extracted from the Canadian Open Neuroscience Platform, a national initiative for open neuroscience. The recommendations provided by our system (AUC$=0.83$) are significantly better than chance and outperform recommendations made by domain experts using their previous knowledge as well as pipeline and dataset descriptions (AUC$=0.63$). In particular, domain experts often neglect low-level technical aspects of a pipeline-dataset interaction, such as the level of pre-processing, which are captured by a provenance-based system. We conclude that provenance-based pipeline and dataset recommenders are feasible and beneficial to the sharing and usage of open-science resources. Future work will focus on the collection of more comprehensive provenance traces, and on deploying the system in production.

==> bibliography.tex <==
@article{li2016first,
  title={The first step for neuroimaging data analysis: {DICOM} to {NIfTI} conversion},
  author={Li, Xiangrui and Morgan, Paul S and Ashburner, John and Smith, Jolinda and Rorden, Christopher},
  journal={Journal of neuroscience methods},
  volume={264},
  pages={47--56},
  year={2016},
  publisher={Elsevier}
}

@url{conp,
 year = {Accessed: 23 Jul, 2021},
 title = {Canadian Open Neuroscience Platform},
 howpublished = {http://portal.conp.ca}
}

@article{wilkinson2016fair,
  title={The {FAIR} Guiding Principles for scientific data management and stewardship},
  author={Wilkinson, Mark D and Dumontier, Michel and Aalbersberg, IJsbrand Jan and Appleton, Gabrielle and Axton, Myles and Baak, Arie and Blomberg, Niklas and Boiten, Jan-Willem and da Silva Santos, Luiz Bonino and Bourne, Philip E and others},
  journal={Scientific data},
  volume={3},
  number={1},
  pages={1--9},
  year={2016},
  publisher={Nature Publishing Group}
}

@article{gardner2008neuroscience,
  title={The neuroscience information framework: a data and knowledge environment for neuroscience},
  author={Gardner, Daniel and Akil, Huda and Ascoli, Giorgio A and Bowden, Douglas M and Bug, William and Donohue, Duncan E and Goldberg, David H and Grafstein, Bernice and Grethe, Jeffrey S and Gupta, Amarnath and others},
  journal={Neuroinformatics},
  volume={6},
  number={3},
  pages={149--160},
  year={2008},
  publisher={Springer}
}


@article{kennedy2016nitrc,
  title={The {NITRC} image repository},
  author={Kennedy, David N and Haselgrove, Christian and Riehl, Jon and Preuss, Nina and Buccigrossi, Robert},
  journal={NeuroImage},
  volume={124},
  pages={1069--1073},
  year={2016},
  publisher={Elsevier}
}


@article{markiewicz2021openneuro,
  title={{OpenNeuro}: An open resource for sharing of neuroimaging data},
  author={Markiewicz, Christopher J and Gorgolewski, Krzysztof Jacek and Feingold, Franklin and Blair, Ross and Halchenko, Yaroslav O and Miller, Eric and Hardcastle, Nell and Wexler, Joe and Esteban, Oscar and Goncalves, Mathias and others},
  journal={bioRxiv},
  year={2021},
  publisher={Cold Spring Harbor Laboratory}
}
@misc{oracle,
    title = {Oracle Machine Learning for {P}ython User's Guide, Release 1.0},  
    Author = {David McDermid},
    Contributors = {Mark Hornick, Mandeep Kaur, Sherry Lamonica, Feng Li, Boriana Milenova, Venkatanathan Varadarajan , Andi Wang, Qin Wang, Yu Xiang},
    howpublished = {\url{https://docs.oracle.com/en/database/oracle/machine-learning/oml4py/1/mlpug/algoritm-selection.html#GUID-C7A22403-6F4F-4C94-B193-220D0DCC2722}},
}


@article{bids,
  title={The brain imaging data structure, a format for organizing and describing outputs of neuroimaging experiments},
  author={Gorgolewski, Krzysztof J and Auer, Tibor and Calhoun, Vince D and Craddock, R Cameron and Das, Samir and Duff, Eugene P and Flandin, Guillaume and Ghosh, Satrajit S and Glatard, Tristan and Halchenko, Yaroslav O and others},
  journal={Scientific data},
  volume={3},
  number={1},
  pages={1--9},
  year={2016},
  publisher={Nature Publishing Group}
}


@inproceedings{missier2013w3c,
  title={The W3C PROV family of specifications for modelling provenance metadata},
  author={Missier, Paolo and Belhajjame, Khalid and Cheney, James},
  booktitle={Proceedings of the 16th International Conference on Extending Database Technology},
  pages={773--776},
  year={2013}
}

@misc{https://doi.org/10.25495/7gxk-rd71,
  doi = {10.25495/7GXK-RD71},
  howpublished = {https://www.zenodo.org/},
  author = {{European Organization For Nuclear Research} and {OpenAIRE}},
  keywords = {FOS: Physical sciences, Publication, Dataset},
  language = {en},
  title = {Zenodo},
  publisher = {CERN},
  year = {2013}
}


@article{maumet2016sharing,
  title={Sharing brain mapping statistical results with the neuroimaging data model},
  author={Maumet, Camille and Auer, Tibor and Bowring, Alexander and Chen, Gang and Das, Samir and Flandin, Guillaume and Ghosh, Satrajit and Glatard, Tristan and Gorgolewski, Krzysztof J and Helmer, Karl G and others},
  journal={Scientific data},
  volume={3},
  number={1},
  pages={1--15},
  year={2016},
  publisher={Nature Publishing Group}
}

@misc{gitannex,
 author = {Joey Hess},
 title = { git-annex },
 Operating_systems = {Linux,FreeBSD,Android,OS X, Windows},
 year = {Accessed 23 Jul, 2021},
 Size = {44.2 MB},
 Type = {File synchronization},
 License ={GPL3+, AGPL3+},
 howpublished = {https://git-annex.branchable.com/}
 }
 

@misc{datalad2021,
 year = {2021},
 title = {DataLad version 0.14.6},
 howpublished = {https://doi.org/10.5281/zenodo.5034875}
}


@misc{UnitedNationsGeneralAssembly,
 author = {United Nations General Assembly},
 year = {2015},
 title = {Sustainable Development Goals},
 url = {\url{https://sustainabledevelopment.un.org/}}
}

@article{NeuroimagingDataModel,
  title={Sharing brain mapping statistical results with the neuroimaging data model},
  author={Maumet, Camille and Auer, Tibor and Bowring, Alexander and Chen, Gang and Das, Samir and Flandin, Guillaume and Ghosh, Satrajit and Glatard, Tristan and Gorgolewski, Krzysztof J and Helmer, Karl G and others},
  journal={Scientific data},
  volume={3},
  number={1},
  pages={1--15},
  year={2016},
  publisher={Nature Publishing Group}
}

@misc{DATSDocumentation,
 author = { Philippe Rocca-Serra and Alejandra Gonzalez-Beltran. },
 year = {2016},
 title = {{bioCADDIE DATS}'s documentation},
 howpublished = {https://datatagsuite.github.io/docs/html}
}

@misc{NIMHDataArchive,
 author = {National Institute of Mental Health },
 title = {NIMH Data Archive},
 url = {\url{https://nda.nih.gov/}}
}



@article{sansone2017dats,
  title={{DATS}, the data tag suite to enable discoverability of datasets},
  author={Sansone, Susanna-Assunta and Gonzalez-Beltran, Alejandra and Rocca-Serra, Philippe and Alter, George and Grethe, Jeffrey S and Xu, Hua and Fore, Ian M and Lyle, Jared and Gururaj, Anupama E and Chen, Xiaoling and others},
  journal={Scientific data},
  volume={4},
  number={1},
  pages={1--8},
  year={2017},
  publisher={Nature Publishing Group}
}





@article{botvinik2020variability,
  title={Variability in the analysis of a single neuroimaging dataset by many teams},
  author={Botvinik-Nezer, Rotem and Holzmeister, Felix and Camerer, Colin F and Dreber, Anna and Huber, Juergen and Johannesson, Magnus and Kirchler, Michael and Iwanir, Roni and Mumford, Jeanette A and Adcock, R Alison and others},
  journal={Nature},
  pages={1--7},
  year={2020},
  publisher={Nature Publishing Group}
}
@book{rajaraman2011mining,
  title={Mining of massive datasets},
  author={Rajaraman, Anand and Ullman, Jeffrey David},
  year={2011},
  publisher={Cambridge University Press}
}
@article{koren2009matrix,
  title={Matrix factorization techniques for recommender systems},
  author={Koren, Yehuda and Bell, Robert and Volinsky, Chris},
  journal={Computer},
  volume={42},
  number={8},
  pages={30--37},
  year={2009},
  publisher={IEEE}
}
@inproceedings{hu2008collaborative,
  title={Collaborative filtering for implicit feedback datasets},
  author={Hu, Yifan and Koren, Yehuda and Volinsky, Chris},
  booktitle={2008 Eighth IEEE International Conference on Data Mining},
  pages={263--272},
  year={2008},
  organization={Ieee}
}
@article{gorgolewski2017openneuro,
  title={OpenNeuro—a free online platform for sharing and analysis of neuroimaging data},
  author={Gorgolewski, Krzysztof and Esteban, Oscar and Schaefer, Gunnar and Wandell, Brian and Poldrack, Russell},
  journal={Organization for human brain mapping. Vancouver, Canada},
  volume={1677},
  number={2},
  year={2017}
}
@article{kiar2019serverless,
  title={A serverless tool for platform agnostic computational experiment management},
  author={Kiar, Gregory and Brown, Shawn T and Glatard, Tristan and Evans, Alan C},
  journal={Frontiers in neuroinformatics},
  volume={13},
  pages={12},
  year={2019},
  publisher={Frontiers}
}
@article{glatard2018boutiques,
  title={Boutiques: a flexible framework to integrate command-line applications in computing platforms},
  author={Glatard, Tristan and Kiar, Gregory and Aumentado-Armstrong, Tristan and Beck, Natacha and Bellec, Pierre and Bernard, R{\'e}mi and Bonnet, Axel and Brown, Shawn T and Camarasu-Pop, Sorina and Cervenansky, Fr{\'e}d{\'e}ric and others},
  journal={GigaScience},
  volume={7},
  number={5},
  pages={giy016},
  year={2018},
  publisher={Oxford University Press}
}
@article{bokde2015matrix,
  title={Matrix factorization model in collaborative filtering algorithms: A survey},
  author={Bokde, Dheeraj and Girase, Sheetal and Mukhopadhyay, Debajyoti},
  journal={Procedia Computer Science},
  volume={49},
  pages={136--146},
  year={2015},
  publisher={Elsevier}
}
@inproceedings{bell2007improved,
  title={Improved neighborhood-based collaborative filtering},
  author={Bell, Robert M and Koren, Yehuda},
  booktitle={KDD cup and workshop at the 13th ACM SIGKDD international conference on knowledge discovery and data mining},
  pages={7--14},
  year={2007},
  organization={Citeseer}
}
@article{rossi2016syntactic,
  title={A SYNTACTIC AND SEMANTIC VIEW OF BIG DATA},
  author={Rossi, Rog{\'e}rio and Hirama, Kechi},
  year={2016}
}
@article{vincent2016minc,
  title={MINC 2.0: a flexible format for multi-modal images},
  author={Vincent, Robert D and Neelin, Peter and Khalili-Mahani, Najmeh and Janke, Andrew L and Fonov, Vladimir S and Robbins, Steven M and Baghdadi, Leila and Lerch, Jason and Sled, John G and Adalat, Reza and others},
  journal={Frontiers in neuroinformatics},
  volume={10},
  pages={35},
  year={2016},
  publisher={Frontiers}
}
@article{larobina2014medical,
  title={Medical image file formats},
  author={Larobina, Michele and Murino, Loredana},
  journal={Journal of digital imaging},
  volume={27},
  number={2},
  pages={200--206},
  year={2014},
  publisher={Springer}
}
@article{smith2002fast,
  title={Fast robust automated brain extraction},
  author={Smith, Stephen M},
  journal={Human brain mapping},
  volume={17},
  number={3},
  pages={143--155},
  year={2002},
  publisher={Wiley Online Library}
}
@article{la2021evaluating,
  title={Evaluating recommender systems for {AI}-driven biomedical informatics},
  author={La Cava, William and Williams, Heather and Fu, Weixuan and Vitale, Steve and Srivatsan, Durga and Moore, Jason H},
  journal={Bioinformatics},
  volume={37},
  number={2},
  pages={250--256},
  year={2021},
  publisher={Oxford University Press}
}
@article{fecher2014open,
  title={Open science: one term, five schools of thought},
  author={Fecher, Benedikt and Friesike, Sascha},
  journal={Opening science},
  pages={17--47},
  year={2014},
  publisher={Springer, Cham}
}

@incollection{pazzani2007content,
  title={Content-based recommendation systems},
  author={Pazzani, Michael J and Billsus, Daniel},
  booktitle={The adaptive web},
  pages={325--341},
  year={2007},
  publisher={Springer}
}

@article{dinov2014perfect,
  title={The perfect neuroimaging-genetics-computation storm: collision of petabytes of data, millions of hardware devices and thousands of software tools},
  author={Dinov, Ivo D and Petrosyan, Petros and Liu, Zhizhong and Eggert, Paul and Zamanyan, Alen and Torri, Federica and Macciardi, Fabio and Hobel, Sam and Moon, Seok Woo and Sung, Young Hee and others},
  journal={Brain imaging and behavior},
  volume={8},
  number={2},
  pages={311--322},
  year={2014},
  publisher={Springer}
}
@article{koren2015advances,
  title={Advances in collaborative filtering},
  author={Koren, Yehuda and Bell, Robert},
  journal={Recommender systems handbook},
  pages={77--118},
  year={2015},
  publisher={Springer}
}
@article{berrar2019cross,
  title={Cross-validation},
  author={Berrar, Daniel},
  journal={Encyclopedia of bioinformatics and computational biology},
  volume={1},
  pages={542--545},
  year={2019},
  publisher={Academic}
}
@article{powers2007evaluation,
  title={Evaluation: From precision, recall and F-factor to ROC, informedness, markedness \& correlation (Tech. Rep.)},
  author={Powers, DM},
  journal={Adelaide, Australia},
  year={2007}
}
@inproceedings{lamprecht2010synthesis,
  title={Synthesis-based loose programming},
  author={Lamprecht, Anna-Lena and Naujokat, Stefan and Margaria, Tiziana and Steffen, Bernhard},
  booktitle={2010 Seventh International Conference on the Quality of Information and Communications Technology},
  pages={262--267},
  year={2010},
  organization={IEEE}
}
@inproceedings{naujokat2012loose,
  title={Loose programming with PROPHETS},
  author={Naujokat, Stefan and Lamprecht, Anna-Lena and Steffen, Bernhard},
  booktitle={International Conference on Fundamental Approaches to Software Engineering},
  pages={94--98},
  year={2012},
  organization={Springer}
}

@article{lamprecht2013user,
  title={User-level workflow design},
  author={Lamprecht, Anna-Lena},
  journal={Lecture Notes in Computer Science},
  volume={8311},
  year={2013},
  publisher={Springer}
}

@article{ison2013edam,
  title={EDAM: an ontology of bioinformatics operations, types of data and identifiers, topics and formats},
  author={Ison, Jon and Kala{\v{s}}, Mat{\'u}{\v{s}} and Jonassen, Inge and Bolser, Dan and Uludag, Mahmut and McWilliam, Hamish and Malone, James and Lopez, Rodrigo and Pettifer, Steve and Rice, Peter},
  journal={Bioinformatics},
  volume={29},
  number={10},
  pages={1325--1332},
  year={2013},
  publisher={Oxford University Press}
}
@article{palmblad2019automated,
  title={Automated workflow composition in mass spectrometry-based proteomics},
  author={Palmblad, Magnus and Lamprecht, Anna-Lena and Ison, Jon and Schw{\"a}mmle, Veit},
  journal={Bioinformatics},
  volume={35},
  number={4},
  pages={656--664},
  year={2019},
  publisher={Oxford University Press}
}
@article{gil2010wings,
  title={Wings: Intelligent workflow-based design of computational experiments},
  author={Gil, Yolanda and Ratnakar, Varun and Kim, Jihie and Gonzalez-Calero, Pedro and Groth, Paul and Moody, Joshua and Deelman, Ewa},
  journal={IEEE Intelligent Systems},
  volume={26},
  number={1},
  pages={62--72},
  year={2010},
  publisher={IEEE}
}
@article{kumar2021tool,
  title={Tool recommender system in {G}alaxy using deep learning},
  author={Kumar, Anup and Rasche, Helena and Gr{\"u}ning, Bj{\"o}rn and Backofen, Rolf},
  journal={GigaScience},
  volume={10},
  number={1},
  pages={giaa152},
  year={2021},
  publisher={Oxford University Press}
}

@inproceedings{tornede2019algorithm,
  title={Algorithm selection as recommendation: From collaborative filtering to dyad ranking},
  author={Tornede, Alexander and Wever, Marcel and H{\"u}llermeier, Eyke},
  booktitle={CI Workshop, Dortmund},
  year={2019}
}

@article{vartak2017meta,
  title={A meta-learning perspective on cold-start recommendations for items},
  author={Vartak, Manasi and Thiagarajan, Arvind and Miranda, Conrado and Bratman, Jeshua and Larochelle, Hugo},
  year={2017}
}
@inproceedings{tornede2020extreme,
  title={Extreme algorithm selection with dyadic feature representation},
  author={Tornede, Alexander and Wever, Marcel and H{\"u}llermeier, Eyke},
  booktitle={International Conference on Discovery Science},
  pages={309--324},
  year={2020},
  organization={Springer}
}


@article{schafer2018dyad,
  title={Dyad ranking using Plackett--Luce models based on joint feature representations},
  author={Sch{\"a}fer, Dirk and H{\"u}llermeier, Eyke},
  journal={Machine Learning},
  volume={107},
  number={5},
  pages={903--941},
  year={2018},
  publisher={Springer}
}





